Exploring the Learning Difficulty of Data Theory and Measure

As learning difficulty is crucial for machine learning (e.g., difficulty-based weighting learning strategies), previous literature has proposed a number of learning difficulty measures. However, no comprehensive investigation for learning difficulty is available to date, resulting in that nearly all existing measures are heuristically defined without a rigorous theoretical foundation. In addition, there is no formal definition of easy and hard samples even though they are crucial in many studies. This study attempts to conduct a pilot theoretical study for learning difficulty of samples. First, a theoretical definition of learning difficulty is proposed on the basis of the bias-variance trade-off theory on generalization error. Theoretical definitions of easy and hard samples are established on the basis of the proposed definition. A practical measure of learning difficulty is given as well inspired by the formal definition. Second, the properties for learning difficulty-based weighting strategies are explored. Subsequently, several classical weighting methods in machine learning can be well explained on account of explored properties. Third, the proposed measure is evaluated to verify its reasonability and superiority in terms of several main difficulty factors. The comparison in these experiments indicates that the proposed measure significantly outperforms the other measures throughout the experiments.

==> Experiment.tex <==
\section{Experiments}
As previously mentioned, learning difficulty is heavily determined by the data quality, margin, uncertainty, and imbalance. Therefore, four different scenarios are designed to evaluate the effectiveness of the proposed measurements.

\subsection{Measurement under Noise Detection}
Two benchmark image classification data sets~\cite{b33}, namely, CIFAR10 and CIFAR100, are used. There are 10 classes in CIFAR10 and 100 classes in CIFAR100. On both sets, there are 50,000 images for training and 10,000 images for testing. As only noise detection is explored. the test images are used as the validation data. In this scenario, noises contain two types. The first type is noisy labels ($y$), while the second consists of noisy images ($x$). The competing methods are as follows:
\begin{itemize} 
    \item \textbf{Loss}. The losses for each sample in the epoch with the highest validation accuracy are used for measurement. 
    \item \textbf{Average loss (AveLoss)}. The average values of losses of the last 100 epochs are used for measurement. 
    \item \textbf{O2UNet~\cite{b17}}. As previously introduced, this method adopts a cyclical training procedure and the average loss of each sample in the procedure is used.
    \item \textbf{MentorNet~\cite{b22}}. This method pertaining to curriculum learning, uses the output weights of the teacher network with the highest accuracy on the validation set to present the possibility of being correct. A smaller weight indicates the sample is more difficult to learn.
    \item \textbf{Co-teaching~\cite{b21}}. Two networks are trained. For each sample, the smaller one of the two losses given by the two networks is regarded as the learning difficulty.
    \item \textbf{Variance of gradients (VOG)~\cite{b6}}. This method relies on the variances of the gradient norms of each sample cross different training epochs. A high VOG value indicates a large difficulty for a sample.
    \item \textbf{Our proposed method GELD}. The detailed steps are presented in Algorithm 1.
\end{itemize}

\begin{figure*}[htbp]
\centering
\includegraphics[scale=0.36]{CIFAR10.pdf}
\caption{The F1 scores ($\%$) of the competing methods on CIFAR10 under different sub-types and rates of label noises.}
\label{fig5}
\end{figure*}

In the methods of Loss, AveLoss, O2UNet, VOG, and our GELD, ResNet-34~\cite{b38} is used as the base network. The hyper-parameters of ResNet-34 used in~\cite{b38} are followed. Specifically, the batch-size is 128, the SGD optimizer has a momentum of 0.9, and the weight decay is 1e-4. The learning rate of the first 40 epochs is 0.1 and is multiplied by 0.1 for every 40 epochs. Each model is learned for 200 epochs. The default settings of MentorNet and Co-teaching are borrowed from the corresponding papers~\cite{b22,b21}. O2UNet and VOG contain specific hyper-parameters other than those of ResNet-34. These parameters follow the setting in the original paper~\cite{b6,b17}. In our GELD,
$K$ and $M$ are set as 5 and 6 respectively, for GELD, except for the part \textit{E} (the discussion of the impact of $(K,M)$ value). The tuning factor $\mu$ of GELD is set as 1.

Let $v$ be the noise rate. The result evaluation scheme used for O2UNet~\cite{b17} is followed. In each method, the top-$50000*v*r$ samples are selected as its detected noisy samples according to its estimated difficulties, where $r \in \lbrace 0.8, 0.9, 1, 1.1, 1.2\rbrace$. Then, the whole detection is repeated three times for each method and the average F1 values on the detection results are calculated and compared. A high F1 value indicates a good performance in noisy label detection and thus the learning difficulty measurement. 

\subsubsection{Noisy label detection}
\indent

Two sub-types of noises are used, namely, symmetric and pair-flip. The symmetric noise describes mislabeling to each other classes of equal possibility. In pair-flip, labelers may make mistakes only within very similar class. The noise rate is set as $20\%$, $40\%$, and $60\%$, respectively. The detailed noise setting in \cite{b21} is followed. 

 Figs. \ref{fig5} and \ref{fig6} show the detection performances of the competing method on CIFAR10 and CIFAR100, respectively. Our proposed approach GELD achieves the highest F1 values in most cases. Although O2UNet outperforms GELD under the symmetric noise sub-type on CIFAR100 (Figs. \ref{fig6}(a), (b) and (c)), its performances are quite poor under the pair-flip noises. The performance of the widely-used method Loss is poor and it achieves the worst F1 scores in several cases. Loss is not an ideal measurement for the easy and hard samples even though it does not require additional computational cost.


In our approach GELD, $\mu$ can be tuned. Table \ref{tab1} shows the performance variations of GLED under the pair-flip noise sub-type and different values of $\mu$ in Eq.~(\ref{29}). When the value is larger than one, higher F1 values are achieved. These results reveal the importance of the variance term during the evaluation of the learning difficulty. 


\renewcommand{\arraystretch}{1.1}
\begin{table}[h]
\begin{center}
\begin{minipage}{250pt}
\caption{$F1$ scores (\%) of GELD under various values of $\mu$.}\label{tab1}%
  \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
   &$\mu$ & 0.5 & 0.75 & 1 & 1.25 & 1.5 & 2\\
    \midrule
     \multirow{3}*{\rotatebox{90}{CIFAR10}} &$20\%$ &   90.48 & 92.01 & 93.67 & 93.99 & 94.83& 95.06\\
    \cline{2-8} & $40\%$ & 93.95 & 93.99 & 96.03 & 96.00 & 96.00 & 95.39\\
    \cline{2-8} & $60\%$ & 91.60 & 92.47 & 95.80 & 95.67 & 95.52 & 94.99\\
  \bottomrule
    \midrule
     \multirow{3}*{\rotatebox{90}{CIFAR100}} &$20\%$ &   89.74 & 90.00 & 90.50 & 90.71 & 91.00 & 91.67\\
    \cline{2-8} & $40\%$ & 90.04 & 91.39 & 91.51& 92.00 & 92.33 & 92.97\\
    \cline{2-8} & $60\%$ & 90.33 & 91.05 & 91.39 & 91.49 & 92.41 & 93.22\\
  \bottomrule
\end{tabular}
\end{minipage}
\end{center}
\end{table}


\begin{figure*}[ht]
\centering
\includegraphics[scale=0.36]{CIFAR100.pdf}
\caption{The F1 scores ($\%$) of the competing methods on CIFAR100 under different sub-types and rates of label noises.}
\label{fig6}
\end{figure*}


\subsubsection{Noisy image detection}
\indent

In this experiment, salt-and-pepper noises are leveraged~\cite{b40}. The noise is simulated by adding white (salt) or black (pepper) noises into the original RGB images with a parameter of signal-to-noise ratio (SNR). In our experiment, the SNR is set as 0.4 for each image. Fig. \ref{fig7} shows an example for nosiy images with different SNR levels. The noise rate on the whole data is set as $20\%$ and $40\%$, respectively.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.85\textwidth]{4images.jpg}
\caption{Noisy images with different SNR levels.}\vspace{-0.15in}\label{fig7}%
\end{figure}

Fig. \ref{fig8} shows the performances of the competing methods on CIFAR10 and CIFAR100, respectively. The settings of competing methods remain unchanged compared with the label noise experiments. Our method GELD still achieves the highest F1 values under all the noise rates. Few noisy data were detected by methods that rely merely on the loss.

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{SAP.pdf}
\caption{The F1 scores ($\%$) of the competing methods on CIFAR10 and CIFAR100 under different rates of salt-and-pepper noise.}
\label{fig8}\vspace{-0.1in}
\end{figure}


\subsection{Measurement under Small-margin Data Detection}
A sample with a small margin (the distance to the oracle decision boundary) is considered to be hard in learning \cite{b3}. This experiment evaluates a learning difficulty measure in terms of the detection of small-margin samples.

In this experiment, four UCI~\cite{b39} data sets are used, namely, Iris, Mammographic, Haberman, and Abalone. To better construct the ground-truth, only binary classification is considered. Only two categories are selected for both Iris (the ``Setosa" and ``Versicolour" categories) and Abalone (the ``9" and ``10" categories). Mammographic and Haberman contain only two categories. The details of used data in this experiment are presented in Table \ref{tab2}. The classical margin-based learning method SVM~\cite{b32} is used to construct the ground truth, i.e., the small-margin samples. Specifically, the SVM with RBF kernel is used. Two parameters $C$ and $g$ are searched in \{$10^{-3}, 10^{-2}, 10^{-1},1,10,10^{2},10^{3}$\} and \{$10^{-3}, 10^{-2}, 10^{-1},1,10,10^{2},10^{3}$\}, respectively, via five-fold cross-validation. The optimal parameter setting is used and the SVM is trained on the whole training set. Constantly, the margin of each sample is constantly calculated as the ground-truth difficulty. The margin is $yf(x)$ for the sample $x$, while $y$ is the label and $f(x)$ is the output of the kernel SVM. Let $N$ be the \#Instances. The top-$N*v$ samples with small margins are selected as the ground-truth samples to detect.

As the base network ResNet-34 is inappropriate in this experiment, a three-layer perception with the Sigmoid activation function is used as the base network. The number of epoch is set to 10000. Its hyper-parameters are also pursed via five-fold cross-validation. Considering that MentorNet and Co-teaching are quite complex for this scenario, they are not compared in this experiment. The competing methods include Loss, AveLoss, O2UNet, and our GLED. The evaluation criteria and the whole calculate scheme follow the setting in the previous experiments. The value of $v$ is set as 20\%, 40\%, and 60\%, respectively; $r$ is set as one.



\begin{table}
\begin{center}
\begin{minipage}{250pt}
\caption{Details of the four UCI data sets.}\label{tab2}%
  \begin{tabular}{cccc}
    \toprule
    Data set & \#Dimensions & \#Classes & \#Instances\\
    \midrule
    Iris &   4 & 2 & 100\\
    Mammographic &   5 & 2 & 961\\
    Haberman &   3 & 2 & 360 \\
    Abalone &   8 & 2 & 1323\\
  \bottomrule
\end{tabular}
\end{minipage}
\end{center}
\end{table}


The results are shown in Fig. \ref{fig9}. Our approach GELD achieves the highest F1 values on all data sets. In addition, GELD is stable across different $v$s and different data sets. By contrast, the other methods are not stable. 
\begin{figure}
\centering
\includegraphics[scale=0.4]{margin.pdf}
\caption{Histogrames of F1 scores (\%) under various data sets using margin as ground-truth.}\vspace{-0.1in}
\label{fig9}
\end{figure}

\subsection{Measurement under Epistemic Uncertainty Detection}
In this experiment, a data corpus containing epistemic uncertainty is required. An image aesthetic assessment data corpus, namely, AVA benchmark image aesthetic data corpus~\cite{b42}, is then utilized and each photo receives multiple rating scores from multiple different users. The variance of user rating scores of a photo reflects the epistemic uncertainty on the photo using each user as a gold model. A large variance indicates a large uncertainty for a photo. Specifically, the former 50,000 samples in the AVA corpus are downloaded and each sample receives 210 rates on average counting from 1 to 10. We use ResNet-101 as the base network as the image quality of AVA is much higher than CIFAR10 and CIFAR100. Given that the Bayesian Neural Network (BNN)~\cite{b20} is particularly designed for modeling uncertainty, we import BNN as one of the competing methods, and its outputting confidence coefficient is used to detect uncertain photos. Therefore, the competing methods include Loss, AveLoss, O2UNet, BNN, and our GELD.

The top-$50,000*v$ photos with high uncertain scores are taken as the objective samples to detect. The $v$ values are set as 20\%, 40\%, and 60\%. The $r$ value is set as one. In the BNN method, the dropout strategy described in~\cite{b20} is followed. The parameter setting of ResNet-101 reported in~\cite{b38} is adopted. The photos are resized into shape of (3, 192, 192) to fit in the ResNet-101.



\begin{table}
\begin{center}
\begin{minipage}{250pt}
\caption{$F1$ scores (\%) using the variance of scores as standard}\label{tab3}%
  \begin{tabular}{ccccccc}
    \toprule
    Method & Loss & AveLoss & O2UNet & BNN & GELD\\
    \midrule
    $20\%$ &   14.64 & 54.05& 33.27 & 62.71&\textbf{63.96}\\
    $40\%$ &   28.38 & 33.33& 35.67 & 54.30&\textbf{78.39}\\
   $60\%$ &   30.23 & 45.79& 38.20 & 78.21&\textbf{79.11}  \\
  \bottomrule
\end{tabular}
\end{minipage}
\end{center}
\end{table}

Table \ref{tab3} shows the F1 scores of the competing methods in high uncertain sample detection. GELD still performs the best and slightly outperforms BNN. The rest of the three methods poorly perform in this detection task. 
Fig.~\ref{fig10} shows the top-5 high uncertain photos and the top-5 photos detected by our GELD approach. The aforementioned figure (Fig.~\ref{fig11}) also shows the last five photos with small uncertainty and the last five photos detected by our GELD.


\begin{figure}[htbp]
\centering
\includegraphics[scale=0.145]{Top5.png}
\caption{True highest uncertain photos and our detection results. The histograms of user ratings are also presented.}\vspace{-0.1in}
\label{fig10}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.1]{Last5.png}
\caption{True lowest uncertain photos and our detection results. The histograms of user ratings are also presented.}\vspace{-0.1in}
\label{fig11}
\end{figure}



\subsection{Measurement for Imbalance Data}
The long-tail versions of the CIFAR10 and CIFAR100 are used in this experiment. Buda et al.~\cite{b34} compiled a series of data sets under different imbalance ratios. The two data sets under the $20:1$ ratio for CIFAR10 and CIFAR100  are used. There is no ground-truth information for the learning difficulties because the head categories can also contain difficult samples. Consequently, we only plot the histograms of the numbers of hard samples detected by the competing methods in the head and tail categories. The competing methods are Loss, AvgLoss, O2UNet, VOG, and our proposed GLED. The base network and the concerning setting in part \textit{A} are followed.
\indent

\begin{figure}[htbp]
\begin{center}
\begin{minipage}{250pt}
\includegraphics[scale=0.6]{imbalanceCIFAR10.pdf}
\caption{ Histogram of CIFAR10-LT top-$40\%$ detected hard samples.}\label{fig13}%
\end{minipage}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\begin{minipage}{250pt}
\includegraphics[scale=0.6]{imbalanceCIFAR100.pdf}
\caption{ Histogram of CIFAR100-LT top-$40\%$ detected hard samples.}\label{fig13}%
\end{minipage}
\end{center}
\end{figure}

The top-40\% samples detected by each competing methods are regarded as their detected hard samples. Figs. \ref{fig12} and \ref{fig13} show the histograms of the detected hard samples by each method on CIFAR10 and CIFAR100 (the top five head categories and the last five tail categories), respectively. All the competing methods identically behave on the tail categories on both data corpora. This condition is reasonable and accords well with the primary motivation for imbalance learning that samples in tail categories are hard to learn. There are slight differences between our GELD and other competing methods on the head categories. The numbers of hard samples detected by GELD are larger than those of other methods, which is reasonable because head categories still contain hard samples.

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.4]{NoisyTypeBV.pdf}
\caption{Histograms of bias and variance values calculated by GELD under different types of label noise ($v = 40\%$).}
\label{fig14}\vspace{-0.2in}
\end{figure}

\subsection{Discussion}
\indent

The above experiments on the four scenarios, namely, noise detection, small-margin sample detection, uncertain sample detection, and hard sample detection in imbalance learning, verify the superiority of the proposed GELD approach over existing classical and state-of-the-art methods. As previously introduced, the primary difference between GELD and many existing methods lies in that GELD explicitly considers variances. Fig. \ref{fig14} shows the histograms of the bias values and the variance values achieved by GELD on clean samples and label noisy samples under both pair-flip and symmetric noise types on CIFAR10. The variance values between clean and noisy samples are also considerably distinct as shown in Figs. \ref{fig14} (b) and (d), which demonstrates the usefulness of the variance term utilized in our GELD method. In addition, the difference between the histograms of noisy and clean samples under the pair-flip noises is trivial, which explains the poor performances of the loss-based methods such as O2UNet.


Although good results are achieved, GELD is only an appropriation for theoretical difficulty in Definition 1. We evaluate the robustness of the method in terms of the variations on the two key parameters, namely, $K$ and $M$. Table \ref{tab4} shows the performances of pair-flip noise detection ($r=1$) on CIFAR10 and CIFAR100. The results show that the performances of GELD are stable when the value of $(K,M)$ is set in \{(4, 5), (5, 6), (5, 8), (5, 10)\}.

\renewcommand{\arraystretch}{1.1}
\begin{table}
\begin{center}
\begin{minipage}{250pt}
\caption{$F1$ scores (\%) with various values of $K*M$.}
  \label{tab4}
  \begin{tabular}{cccccc}
    \toprule
   &$K*M$ &20 (4$\times 5$)& 30 ($5\times 6$) &40 ($5\times 8$) &  50 ($5\times 10$) \\
    \midrule
     \multirow{3}*{\rotatebox{90}{CIFAR10}} & $20\%$ & 96.83&  97.51 & 96.91 & 97.04\\
    \cline{2-6} & $40\%$ &94.12 &  95.77& 96.10&  96.34\\
     \cline{2-6} & $60\%$ & 94.81 &  95.82& 94.95 & 95.34 \\
  \midrule
    \midrule
     \multirow{3}*{\rotatebox{90}{CIFAR100}}  & $20\%$ & 90.36 & 91.00 & 92.67&  91.46\\
     \cline{2-6} & $40\%$ & 91.78& 92.48 & 91.86& 91.04 \\
     \cline{2-6} & $60\%$ & 90.02& 92.00& 91.17&  90.89\\
  \bottomrule
\end{tabular}
\end{minipage}
\end{center}
\end{table}

 We are interested in whether a simple model can also obtain better results. A simple network, namely, AlexNet~\cite{b35}, is used as the basic leaner in pair-flip noisy label. The base network and setting of other methods follow the previous setting of the corresponding experiments in part \textit{A}. The training setting of AlexNet in~\cite{b43} is followed, and the output-size is modified into 100 while training CIAFR100. The results are shown in Table \ref{tab5}. GELD (AlexNet) is inferior to GELD (ResNet-34). However, it is comparable to Co-teaching and outperforms the rest of the methods.
 
 
 
\begin{table}
\begin{center}
\begin{minipage}{250pt}
\caption{$F1$ scores (\%) of the competing methods plus GELD using AlexNet as base model.}
  \label{tab5}
  \begin{tabular}{cccccccc}
    \toprule
    Method &\multicolumn{3}{c}{CIFAR10} & \multicolumn{3}{c}{CIFAR100}\\
    \midrule
    Label noise rate & $20\%$ & $40\%$& $60\%$& $20\%$& $40\%$& $60\%$\\
    \midrule
    GELD (ResNet-34) &{97.51} &{95.77}&{95.82}&{91.00}&{92.48}&{92.00}\\
    O2UNet & 92.31&80.76&33.69&61.29&54.03&46.98\\
    Co-teaching& 92.63&89.45&58.02&86.22&89.77&88.90\\
    MentorNet& 88.02&67.96&47.14&73.00&51.49&60.09\\
    AveLoss & 81.39&79.23&51.98&77.38&74.18&79.17\\
    Loss& 76.69&76.12&50.53&75.29&74.15&79.75\\
    GELD (AlexNet)& 82.58&88.77&83.54&82.96&86.51&84.39\\
  \bottomrule
\end{tabular}
\end{minipage}
\end{center}
\end{table}


\begin{table}
\begin{center}
\begin{minipage}{185pt}
\caption{Time cost of different complex methods.}
  \label{tab6}
  \begin{tabular}{cc}
    \toprule
    Method & Time cost (hours)\\
    \midrule
    O2UNet & 7.95\\
    GELD (1 GPU) & 11.11\\
    GELD (2 GPUs) & 5.67\\
    GELD (3 GPUs) & 3.71\\
    GELD (4 GPUs) & 2.83 \\
  \bottomrule
\end{tabular}
\end{minipage}
\end{center}
\end{table}
The computational cost of GELD is relatively high as $K*M$ models should be trained. However, the task can be performed in parallel. Four NVIDIA GeForce RTX 3090 GPUs are used in our experiments. The average time costs for our GELD using different number of GPUs on CIFAR10 using ResNet-34 as base network are shown in Table \ref{tab6}. The settings follow the pair-flip label noise experiments' in part \textit{A} with $(K, M)$ is set as (5, 6). The time consumption is considerably reduced when GELD is run on more GPUs in parallel. The time cost of O2UNet is also large. More over, O2UNet cannot be performed in parallel.

==> model5-names.tex <==
%%
%% This is file `model5-names.bst'  (Version 2.0),
%% 
%% Copyright 2009-2012 Elsevier Ltd
%% 
%% This file is part of the 'Elsarticle Bundle'.
%% ---------------------------------------------
%% 
%% It may be distributed under the conditions of the LaTeX Project Public
%% License, either version 1.2 of this license or (at your option) any
%% later version.  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%%
%% $Id: model5-names.bst 214 2012-10-22 07:34:19Z rishi $
%%
%% $URL: http://lenova.river-valley.com/svn/elsbst/trunk/New-Model-5/model5-names.bst $
%%
%%

ENTRY
  { address
    author
    booktitle
    chapter
    collaboration
    edition
    editor
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    volume
    year
    url
    doi
    eprint
    pubmed
  }
  {}
  { label extra.label sort.label short.list }

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

STRINGS { urlprefix doiprefix eprintprefix pubmedprefix }

FUNCTION {init.web.variables}
{
 "\URLprefix "     'urlprefix :=
 "\DOIprefix"      'doiprefix :=
 "\ArXivprefix  "   'eprintprefix :=
 "\Pubmedprefix "  'pubmedprefix :=
}

FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}
STRINGS { s t}
FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { " " * write$ }
    { output.state after.block =
        { add.period$ write$
          newline$
          "\newblock " write$
        }
        { output.state before.all =
            'write$
            { add.period$ " " * write$ }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}
FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}
FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}
FUNCTION {fin.entry}
{ add.period$
  write$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}
FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
        'skip$
        { after.sentence 'output.state := }
      if$
    }
  if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {date.block}
{
  new.block
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}
FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}
FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}
FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}
FUNCTION {emphasize}
{ duplicate$ empty$
    { pop$ "" }
    { "{\it " swap$ * "\/}" * }
  if$
}
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
 % Here are the language-specific definitions for explicit words.
 % Each function has a name bbl.xxx where xxx is the English word.
 % The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "\&"}

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "eds." }

FUNCTION {bbl.editor}
{ "ed." }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "ed." }

FUNCTION {bbl.volume}
{ "volume" }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "number" }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "pp." }

FUNCTION {bbl.page}
{ "p." }

FUNCTION {bbl.chapter}
{ "chapter" }

FUNCTION {bbl.techrep}
{ "Technical Report" }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "Ph.D. thesis" }

FUNCTION {bbl.first}
{ "1st" }

FUNCTION {bbl.second}
{ "2nd" }

FUNCTION {bbl.third}
{ "3rd" }

FUNCTION {bbl.fourth}
{ "4th" }

FUNCTION {bbl.fifth}
{ "5th" }

FUNCTION {bbl.st}
{ "st" }

FUNCTION {bbl.nd}
{ "nd" }

FUNCTION {bbl.rd}
{ "rd" }

FUNCTION {bbl.th}
{ "th" }

MACRO {jan} {"January"}

MACRO {feb} {"February"}

MACRO {mar} {"March"}

MACRO {apr} {"April"}

MACRO {may} {"May"}

MACRO {jun} {"June"}

MACRO {jul} {"July"}

MACRO {aug} {"August"}

MACRO {sep} {"September"}

MACRO {oct} {"October"}

MACRO {nov} {"November"}

MACRO {dec} {"December"}

FUNCTION {eng.ord}
{ duplicate$ "1" swap$ *
  #-2 #1 substring$ "1" =
     { bbl.th * }
     { duplicate$ #-1 #1 substring$
       duplicate$ "1" =
         { pop$ bbl.st * }
         { duplicate$ "2" =
             { pop$ bbl.nd * }
             { "3" =
                 { bbl.rd * }
                 { bbl.th * }
               if$
             }
           if$
          }
       if$
     }
   if$
}

MACRO {acmcs} {"ACM Comput. Surv."}

MACRO {acta} {"Acta Inf."}

MACRO {cacm} {"Commun. ACM"}

MACRO {ibmjrd} {"IBM J. Res. Dev."}

MACRO {ibmsj} {"IBM Syst.~J."}

MACRO {ieeese} {"IEEE Trans. Software Eng."}

MACRO {ieeetc} {"IEEE Trans. Comput."}

MACRO {ieeetcad}
 {"IEEE Trans. Comput. Aid. Des."}

MACRO {ipl} {"Inf. Process. Lett."}

MACRO {jacm} {"J.~ACM"}

MACRO {jcss} {"J.~Comput. Syst. Sci."}

MACRO {scp} {"Sci. Comput. Program."}

MACRO {sicomp} {"SIAM J. Comput."}

MACRO {tocs} {"ACM Trans. Comput. Syst."}

MACRO {tods} {"ACM Trans. Database Syst."}

MACRO {tog} {"ACM Trans. Graphic."}

MACRO {toms} {"ACM Trans. Math. Software"}

MACRO {toois} {"ACM Trans. Office Inf. Syst."}

MACRO {toplas} {"ACM Trans. Progr. Lang. Syst."}

MACRO {tcs} {"Theor. Comput. Sci."}

FUNCTION {bibinfo.check}
{ swap$
  duplicate$ missing$
    {
      pop$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ pop$
        }
        { swap$
          "\bibinfo{" swap$ * "}{" * swap$ * "}" *
        }
      if$
    }
  if$
}
FUNCTION {bibinfo.warn}
{ swap$
  duplicate$ missing$
    {
      swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ "empty " swap$ * " in " * cite$ * warning$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
STRINGS  { bibinfo}
INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}{, f.}{, jj}"
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          nameptr #9
          #90 +
          #1 + =
          numnames #9
          #90 +
          > and
            { "others" 't :=
              #1 'namesleft := }
            'skip$
          if$
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " " * bbl.etal *
                }
                {"," *
                  bbl.and
                  space.word * t *
                }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.names.ed}
{
  'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{f.~}{vv~}{ll}{, jj}"
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {

                  " " * bbl.etal *
                }
                {"," *
                  bbl.and
                  space.word * t *
                }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.key}
{ empty$
    { key field.or.null }
    { "" }
  if$
}

FUNCTION {format.authors}
{ author "author" format.names
    duplicate$ empty$ 'skip$
    { collaboration "collaboration" bibinfo.check
      duplicate$ empty$ 'skip$
        { " (" swap$ * ")" * }
      if$
      *
    }
  if$
}


FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
    {
      " " *
      get.bbl.editor
      capitalize
   "(" swap$ * ")" *
      *
    }
  if$
}
FUNCTION {format.note}
{
 note empty$
    { "" }
    { note #1 #1 substring$
      duplicate$ "{" =
        'skip$
        { output.state mid.sentence =
          { "l" }
          { "u" }
        if$
        change.case$
        }
      if$
      note #2 global.max$ substring$ * "note" bibinfo.check
    }
  if$
}

FUNCTION {format.title}
{ title
  duplicate$ empty$ 'skip$
    { "t" change.case$ }
  if$
  "title" bibinfo.check
}
FUNCTION {format.full.names}
{'s :=
 "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}" format.name$
      't :=
      nameptr #1 >
        {
          nameptr #9
          #90 +
          #1 + =
          numnames #9
          #90 +
          > and
            { "others" 't :=
              #1 'namesleft := }
            'skip$
          if$
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " " * bbl.etal *
                }
                {
                  bbl.and
                  space.word * t *
                }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {author.editor.key.full}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.full.names }
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {author.key.full}
{ author empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {editor.key.full}
{ editor empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { editor format.full.names }
  if$
}

FUNCTION {make.full.names}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.full
    { type$ "proceedings" =
        'editor.key.full
        'author.key.full
      if$
    }
  if$
}

FUNCTION {output.bibitem}
{ newline$
  "\bibitem[{" write$
  label write$
  ")" make.full.names duplicate$ short.list =
     { pop$ }
     { * }
   if$
  "}]{" * write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {n.dashify}
{
  't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

FUNCTION {word.in}
{ bbl.in capitalize
  "" *
  " " * }

FUNCTION {format.date}
{ year "year" bibinfo.check duplicate$ empty$
    {
    }
    'skip$
  if$
  extra.label *
  before.all 'output.state :=
  " (" swap$ * ")" *
}
FUNCTION {format.btitle}
{ title "title" bibinfo.check
  duplicate$ empty$ 'skip$
    {
      emphasize
    }
  if$
}
FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}
FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { bbl.volume volume tie.or.space.prefix
      "volume" bibinfo.check * *
      series "series" bibinfo.check
      duplicate$ empty$ 'pop$
        { swap$ bbl.of space.word * swap$
          emphasize * }
      if$
      "volume and number" number either.or.check
    }
  if$
}
FUNCTION {format.number.series}
{ volume empty$
    { number empty$
        { series field.or.null }
        { series empty$
            { number "number" bibinfo.check }
        { output.state mid.sentence =
            { bbl.number }
            { bbl.number capitalize }
          if$
          number tie.or.space.prefix "number" bibinfo.check * *
          bbl.in space.word *
          series "series" bibinfo.check *
        }
      if$
    }
      if$
    }
    { "" }
  if$
}
FUNCTION {is.num}
{ chr.to.int$
  duplicate$ "0" chr.to.int$ < not
  swap$ "9" chr.to.int$ > not and
}

FUNCTION {extract.num}
{ duplicate$ 't :=
  "" 's :=
  { t empty$ not }
  { t #1 #1 substring$
    t #2 global.max$ substring$ 't :=
    duplicate$ is.num
      { s swap$ * 's := }
      { pop$ "" 't := }
    if$
  }
  while$
  s empty$
    'skip$
    { pop$ s }
  if$
}

FUNCTION {convert.edition}
{ extract.num "l" change.case$ 's :=
  s "first" = s "1" = or
    { bbl.first 't := }
    { s "second" = s "2" = or
        { bbl.second 't := }
        { s "third" = s "3" = or
            { bbl.third 't := }
            { s "fourth" = s "4" = or
                { bbl.fourth 't := }
                { s "fifth" = s "5" = or
                    { bbl.fifth 't := }
                    { s #1 #1 substring$ is.num
                        { s eng.ord 't := }
                        { edition 't := }
                      if$
                    }
                  if$
                }
              if$
            }
          if$
        }
      if$
    }
  if$
  t
}

FUNCTION {format.edition}
{ edition duplicate$ empty$ 'skip$
    {
      convert.edition
      output.state mid.sentence =
        { "l" }
        { "t" }
      if$ change.case$
      "edition" bibinfo.check
      " " * bbl.edition *
   "(" swap$ * ")" *
     }
  if$
}
INTEGERS { multiresult }
FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
        { #1 'multiresult := }
        { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}
FUNCTION {format.pages}
{ pages duplicate$ empty$ 'skip$
    { duplicate$ multi.page.check
        {
          bbl.pages swap$
          n.dashify
        }
        {
          bbl.page swap$
        }
      if$
      tie.or.space.prefix
      "pages" bibinfo.check
      * *
     "(" swap$ * ")" *
    }
  if$
}

FUNCTION {format.journal.pages}
{ pages duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$
        { pop$ pop$ format.pages }
        {
          ", " *
          swap$
          n.dashify
          "pages" bibinfo.check
          *
        }
      if$
    }
  if$
}
FUNCTION {format.vol.num.pages}
{ volume field.or.null
  duplicate$ empty$ 'skip$
    {
      "volume" bibinfo.check
    }
  if$
  emphasize
  format.journal.pages
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
        { bbl.chapter }
        { type "l" change.case$
          "type" bibinfo.check
        }
      if$
      chapter tie.or.space.prefix
      "chapter" bibinfo.check
      * *
      pages empty$
        'skip$
        { ". " * format.pages * }
      if$
    }
  if$
}

FUNCTION {format.booktitle}
{
  booktitle "booktitle" bibinfo.check
  emphasize
}
FUNCTION {format.in.ed.booktitle}
{ format.booktitle duplicate$ empty$ 'skip$
    {
      editor "editor" format.names.ed duplicate$ empty$ 'pop$
        {
          " " *
          get.bbl.editor
          capitalize
          "(" swap$ * "), " *
          * swap$
          * }
      if$
      word.in swap$ *
    }
  if$
}
FUNCTION {format.thesis.type}
{ type duplicate$ empty$
    'pop$
    { swap$ pop$
      "t" change.case$ "type" bibinfo.check
    }
  if$
}
FUNCTION {format.tr.number}
{ number "number" bibinfo.check
  type duplicate$ empty$
    { pop$ bbl.techrep }
    'skip$
  if$
  "type" bibinfo.check
  swap$ duplicate$ empty$
    { pop$ "t" change.case$ }
    { tie.or.space.prefix * * }
  if$
}
FUNCTION {format.article.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.book.crossref}
{ volume duplicate$ empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      pop$ word.in
    }
    { bbl.volume
      capitalize
      swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
    }
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.incoll.inproc.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.org.or.pub}
{ 't :=
  ""
  address empty$ t empty$ and
    'skip$
    {
      address "address" bibinfo.check *
      t empty$
        'skip$
        { address empty$
            'skip$
            { ": " * }
          if$
          t *
        }
      if$
    }
  if$
}
FUNCTION {format.publisher.address}
{ publisher "publisher" bibinfo.check format.org.or.pub
}

FUNCTION {format.organization.address}
{ organization "organization" bibinfo.check format.org.or.pub
}

FUNCTION {print.url}
 {url duplicate$ empty$
   { pop$ "" }
   { new.sentence
     urlprefix "\url{" * swap$  * "}" *
   }
   if$
 }

FUNCTION {print.doi}
 {doi duplicate$ empty$
   { pop$ "" }
   { new.sentence
     doiprefix "\doi{" * swap$  * "}" *
   }
   if$
 }

FUNCTION {print.eprint}
 {eprint duplicate$ empty$
   { pop$ "" }
   { new.sentence
     duplicate$ "\href{http://arxiv.org/abs/" swap$ * "}{\tt arXiv:" * swap$ * "}" *
   }
   if$
 }

FUNCTION {print.pubmed}
 {pubmed duplicate$ empty$
   { pop$ "" }
   { new.sentence
     pubmedprefix "\Pubmed{" * swap$  * "}" *
   }
   if$
 }

FUNCTION {webpage}
{ "%Type = Webpage" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  author empty$
  {
    format.title "title" output.check
    new.block
    format.date "year" output.check
    date.block
  }
  {
    format.date "year" output.check
    date.block
    format.title "title" output.check
    new.block
}
  if$
  print.url output
  fin.entry
}

FUNCTION {article}
{ "%Type = Article" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  crossref missing$
    {
      journal
      "journal" bibinfo.check
      emphasize
      "journal" output.check
      ", " *
      format.vol.num.pages output
    }
    { format.article.crossref output.nonnull
      format.pages output
    }
  if$
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  new.block
  format.note output
  fin.entry
}

FUNCTION {book}
{ "%Type = Book" write$
  output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
    }
    { format.authors output.nonnull
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      new.block
      new.sentence
      format.number.series output
      format.edition output
      new.block
      format.publisher.address output
    }
    {
      new.block
      format.book.crossref output.nonnull
    }
  if$
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {booklet}
{ "%Type = booklet" write$
  output.bibitem
  format.authors output
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  howpublished "howpublished" bibinfo.check output
  address "address" bibinfo.check output
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {inbook}
{ "%Type = Inbook" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.number.series output
      format.chapter.pages output
      new.block
      format.publisher.address output
      format.bvolume output
      new.sentence
      format.edition output
    }
    { format.incoll.inproc.crossref output.nonnull
    }
  if$
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}


FUNCTION {incollection}
{ "%Type = Incollection" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.number.series output
      format.chapter.pages output
      new.block
      format.publisher.address output
      format.bvolume output
      new.sentence
      format.edition output
    }
    { format.incoll.inproc.crossref output.nonnull
    }
  if$
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {inproceedings}
{ "%Type = Inproceedings" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.number.series output
      format.pages output
      new.block
      publisher empty$
        { format.organization.address output }
        { organization "organization" bibinfo.check output
          format.publisher.address output
        }
      if$
      format.bvolume output
    }
    { format.incoll.inproc.crossref output.nonnull
    }
  if$
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {conference} { inproceedings }

FUNCTION {manual}
{ "%Type = Manual" write$
  output.bibitem
  format.authors output
  author format.key output
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  organization address new.block.checkb
  organization "organization" bibinfo.check output
  address "address" bibinfo.check output
  format.edition output
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {mastersthesis}
{ "%Type = Masterthesis" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.btitle
  "title" output.check
  new.block
  bbl.mthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {misc}
{ "%Type = Misc" write$
  output.bibitem
  format.authors output
  author format.key output
  format.date "year" output.check
  date.block
  format.title output
  new.block
  howpublished "howpublished" bibinfo.check output
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {phdthesis}
{ "%Type = Phdthesis" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.btitle
  "title" output.check
  new.block
  bbl.phdthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {proceedings}
{ "%Type = Proceedings" write$
  output.bibitem
  format.editors output
  editor format.key output
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  format.bvolume output
  new.sentence
  format.number.series output
  publisher empty$
    { format.organization.address output }
    { organization "organization" bibinfo.check output
      format.publisher.address output
    }
  if$
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {techreport}
{ "%Type = Techreport" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.btitle
  "title" output.check
  new.block
  format.tr.number output.nonnull
  institution "institution" bibinfo.warn output
  address "address" bibinfo.check output
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {unpublished}
{ "%Type = Unpublished" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.block
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note "note" output.check
  fin.entry
}

FUNCTION {default.type} { misc }
READ
FUNCTION {sortify}
{ purify$
  "l" change.case$
}
INTEGERS { len }
FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}
FUNCTION {format.lab.names}
{ 's :=
  "" 't :=
  s #1 "{vv~}{ll}" format.name$
  s num.names$ duplicate$
  #2 >
    { pop$
      " " * bbl.etal *
    }
    { #2 <
        'skip$
        { s #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            {
              " " * bbl.etal *
            }
            { bbl.and space.word * s #2 "{vv~}{ll}" format.name$
              * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {author.key.label}
{ author empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.editor.key.label}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.lab.names }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {editor.key.label}
{ editor empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { editor format.lab.names }
  if$
}

FUNCTION {calc.short.authors}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.label
    { type$ "proceedings" =
        'editor.key.label
        'author.key.label
      if$
    }
  if$
  'short.list :=
}

FUNCTION {calc.label}
{ calc.short.authors
  short.list
  "("
  *
  year duplicate$ empty$
  short.list key field.or.null = or
     { pop$ "" }
     'skip$
  if$
  *
  'label :=
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{ll{ }}{  f{ }}{  jj{ }}"
      format.name$ 't :=
      nameptr #1 >
        {
          nameptr #9
          #90 +
          #1 + =
          numnames #9
          #90 +
          > and
            { "others" 't :=
              #1 'namesleft := }
            'skip$
          if$
          "   "  *
          namesleft #1 = t "others" = and
            { "zzzzz" * }
            { t sortify * }
          if$
        }
        { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}
FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {editor.sort}
{ editor empty$
    { key empty$
        { "to sort, need editor or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { editor sort.format.names }
  if$
}
FUNCTION {presort}
{ calc.label
  label sortify
  "    "
  *
  type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.sort
        'author.sort
      if$
    }
  if$
  #1 entry.max$ substring$
  'sort.label :=
  sort.label
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}
SORT
STRINGS { last.label next.extra }
INTEGERS { last.extra.num number.label }
FUNCTION {initialize.extra.label.stuff}
{ #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'last.extra.num :=
  #0 'number.label :=
}
FUNCTION {forward.pass}
{ last.label label =
    { last.extra.num #1 + 'last.extra.num :=
      last.extra.num int.to.chr$ 'extra.label :=
    }
    { "a" chr.to.int$ 'last.extra.num :=
      "" 'extra.label :=
      label 'last.label :=
    }
  if$
  number.label #1 + 'number.label :=
}
FUNCTION {reverse.pass}
{ next.extra "b" =
    { "a" 'extra.label := }
    'skip$
  if$
  extra.label 'next.extra :=
  extra.label
  duplicate$ empty$
    'skip$
    { "{\natexlab{" swap$ * "}}" * }
  if$
  'extra.label :=
  label extra.label * 'label :=
}
EXECUTE {initialize.extra.label.stuff}
ITERATE {forward.pass}
REVERSE {reverse.pass}
FUNCTION {bib.sort.order}
{ sort.label
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}
ITERATE {bib.sort.order}
SORT
FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{" number.label int.to.str$ * "}" *
  write$ newline$
  "\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi"
  write$ newline$
  "\providecommand{\url}[1]{\texttt{#1}}"
  write$ newline$
  "\providecommand{\href}[2]{#2}"
  write$ newline$
  "\providecommand{\path}[1]{#1}"
  write$ newline$
  "\providecommand{\DOIprefix}{doi:}"
  write$ newline$
  "\providecommand{\ArXivprefix}{arXiv:}"
  write$ newline$
  "\providecommand{\URLprefix}{URL: }"
  write$ newline$
  "\providecommand{\Pubmedprefix}{pmid:}"
  write$ newline$
  "\providecommand{\doi}[1]{\href{http://dx.doi.org/#1}{\path{#1}}}"
  write$ newline$
  "\providecommand{\Pubmed}[1]{\href{pmid:#1}{\path{#1}}}"
  write$ newline$
  "\providecommand{\bibinfo}[2]{#2}"
  write$ newline$
	"\ifx\xfnm\relax \def\xfnm[#1]{\unskip,\space#1}\fi"
  write$ newline$
}
EXECUTE {begin.bib}
EXECUTE {init.state.consts}
EXECUTE {init.web.variables} 
ITERATE {call.type$}
FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}
EXECUTE {end.bib}
%% End of customized bst file
%%
%% End of file `model5-names.bst'.
%%
%% Change log:
%% -----------
%% 22.04.2011
%%
%% 10.08.2012
%%   a. doi, url, eprint, pmid added
%%   b. Bibtype `webpage' defined
%%
%% 30.08.2012
%%   a. collaboration added.
%%


